How to Account for Alternatives When Comparing Effects: Revisiting 'Bringing Education to Afghan Girls'

This paper uses a "principal strata" approach to decompose treatment effects and interpret why a schooling intervention that yielded exceptional initial effects yielded substantially smaller effects in a replication years later. The specific application is a set of 2008 and 2015 replications of an intervention aiming to increase primary education for girls in rural Afghanistan. The intervention offers a new schooling option, and as such, its effects depend on how individuals use alternatives that already exist. The principal strata approach accounts variation in use patterns when comparing effects across the replications. Our findings show that even though the share of girls for whom the intervention would be valuable dropped considerably in 2015 as compared to 2008, the intervention was even more efficaciousness for those who continued to benefit from it.

==> ITT-interactions-2008-mod.tex <==

\begin{table}
\begin{center}
\begin{scriptsize}
\begin{tabular}{l c c c c c c}
\hline
 & 1 & 2 & 3 & 4 & 5 & 6* \\
\hline
Control mean          & $-0.21$  & $-0.23$  & $-0.23$  & $-0.24$  & $-0.23$  & $-0.16$  \\
                      & $(0.12)$ & $(0.14)$ & $(0.14)$ & $(0.14)$ & $(0.13)$ & $(0.16)$ \\
Treatment             & $0.71$   & $0.78$   & $0.79$   & $0.78$   & $0.77$   & $0.58$   \\
                      & $(0.12)$ & $(0.14)$ & $(0.14)$ & $(0.14)$ & $(0.14)$ & $(0.16)$ \\
Child's age           & $0.29$   &          &          &          &          &          \\
                      & $(0.08)$ &          &          &          &          &          \\
Tr. X Child's age     & $0.09$   &          &          &          &          &          \\
                      & $(0.08)$ &          &          &          &          &          \\
HH. head age          &          & $-0.00$  &          &          &          &          \\
                      &          & $(0.00)$ &          &          &          &          \\
Tr. X HH. head age    &          & $0.01$   &          &          &          &          \\
                      &          & $(0.01)$ &          &          &          &          \\
HH. head school       &          &          & $0.03$   &          &          &          \\
                      &          &          & $(0.02)$ &          &          &          \\
Tr. X HH. head school &          &          & $0.02$   &          &          &          \\
                      &          &          & $(0.05)$ &          &          &          \\
HH. head farm.        &          &          &          & $-0.28$  &          &          \\
                      &          &          &          & $(0.31)$ &          &          \\
Tr. X HH. head farm.  &          &          &          & $0.29$   &          &          \\
                      &          &          &          & $(0.31)$ &          &          \\
Land                  &          &          &          &          & $-0.07$  &          \\
                      &          &          &          &          & $(0.05)$ &          \\
Tr. X Land            &          &          &          &          & $-0.06$  &          \\
                      &          &          &          &          & $(0.13)$ &          \\
\hline
N             & $688$    & $689$    & $688$    & $689$    & $689$    & $507$    \\
\hline
\end{tabular}
\end{scriptsize}
\caption{Least squares regression estimates of 2008 sample intention-to-treat and covariate-interaction effects. Outcome is combined math-verbal test score, standardized. Standard errors account for village-level clustering.
 *Model 6 omits Tajik households. }
\label{itt-interactions-2008}
\end{center}
\end{table}


==> ITT-interactions-2008.tex <==

\begin{table}
\begin{center}
\begin{scriptsize}
\begin{tabular}{l c c c c c c}
\hline
 & 1 & 2 & 3 & 4 & 5 & 6* \\
\hline
Control mean          & $-0.21$  & $-0.23$  & $-0.23$  & $-0.24$  & $-0.23$  & $-0.16$  \\
                      & $(0.12)$ & $(0.14)$ & $(0.14)$ & $(0.14)$ & $(0.13)$ & $(0.16)$ \\
Treatment             & $0.71$   & $0.78$   & $0.79$   & $0.78$   & $0.77$   & $0.58$   \\
                      & $(0.12)$ & $(0.14)$ & $(0.14)$ & $(0.14)$ & $(0.14)$ & $(0.16)$ \\
Child's age           & $0.29$   &          &          &          &          &          \\
                      & $(0.08)$ &          &          &          &          &          \\
Tr. X Child's age     & $0.09$   &          &          &          &          &          \\
                      & $(0.08)$ &          &          &          &          &          \\
HH. head age          &          & $-0.00$  &          &          &          &          \\
                      &          & $(0.00)$ &          &          &          &          \\
Tr. X HH. head age    &          & $0.01$   &          &          &          &          \\
                      &          & $(0.01)$ &          &          &          &          \\
HH. head school       &          &          & $0.03$   &          &          &          \\
                      &          &          & $(0.02)$ &          &          &          \\
Tr. X HH. head school &          &          & $0.02$   &          &          &          \\
                      &          &          & $(0.05)$ &          &          &          \\
HH. head farm.        &          &          &          & $-0.28$  &          &          \\
                      &          &          &          & $(0.31)$ &          &          \\
Tr. X HH. head farm.  &          &          &          & $0.29$   &          &          \\
                      &          &          &          & $(0.31)$ &          &          \\
Land                  &          &          &          &          & $-0.07$  &          \\
                      &          &          &          &          & $(0.05)$ &          \\
Tr. X Land            &          &          &          &          & $-0.06$  &          \\
                      &          &          &          &          & $(0.13)$ &          \\
\hline
R$^2$                 & $0.37$   & $0.13$   & $0.15$   & $0.14$   & $0.14$   & $0.09$   \\
Adj. R$^2$            & $0.36$   & $0.13$   & $0.15$   & $0.13$   & $0.14$   & $0.08$   \\
Num. obs.             & $688$    & $689$    & $688$    & $689$    & $689$    & $507$    \\
RMSE                  & $0.03$   & $0.04$   & $0.04$   & $0.04$   & $0.04$   & $0.04$   \\
N Clusters            & $11$     & $11$     & $11$     & $11$     & $11$     & $11$     \\
\hline
\end{tabular}
\end{scriptsize}
\caption{Least squares regression estimates of 2008 sample intention-to-treat and covariate-interaction effects. Outcome is combined math-verbal test score, standardized. Standard errors account for village-level clustering.
 *Model 6 omits Tajik households. }
\label{itt-interactions-2008}
\end{center}
\end{table}


==> ITT-interactions-2015-mod.tex <==

\begin{table}
\begin{center}
\begin{scriptsize}
\begin{tabular}{l c c c c c c c}
\hline
 & 1 & 2 & 3 & 4 & 5 & 6* & 7** \\
\hline
Control mean          & $-0.19$  & $-0.18$  & $-0.20$  & $-0.18$  & $-0.18$  & $-0.21$  & $-0.19$  \\
                      & $(0.10)$ & $(0.12)$ & $(0.12)$ & $(0.12)$ & $(0.12)$ & $(0.13)$ & $(0.13)$ \\
Treatment             & $0.38$   & $0.36$   & $0.38$   & $0.35$   & $0.35$   & $0.38$   & $0.36$   \\
                      & $(0.11)$ & $(0.13)$ & $(0.13)$ & $(0.13)$ & $(0.13)$ & $(0.14)$ & $(0.15)$ \\
Child's age           & $0.26$   &          &          &          &          &          &          \\
                      & $(0.04)$ &          &          &          &          &          &          \\
Tr. X Child's age     & $0.00$   &          &          &          &          &          &          \\
                      & $(0.05)$ &          &          &          &          &          &          \\
HH. head age          &          & $0.00$   &          &          &          &          &          \\
                      &          & $(0.00)$ &          &          &          &          &          \\
Tr. X HH. head age    &          & $0.00$   &          &          &          &          &          \\
                      &          & $(0.00)$ &          &          &          &          &          \\
HH. head school       &          &          & $0.02$   &          &          &          &          \\
                      &          &          & $(0.01)$ &          &          &          &          \\
Tr. X HH. head school &          &          & $-0.00$  &          &          &          &          \\
                      &          &          & $(0.02)$ &          &          &          &          \\
HH. head farm.        &          &          &          & $-0.19$  &          &          &          \\
                      &          &          &          & $(0.11)$ &          &          &          \\
Tr. X HH. head farm.  &          &          &          & $0.07$   &          &          &          \\
                      &          &          &          & $(0.13)$ &          &          &          \\
Land                  &          &          &          &          & $-0.10$  &          &          \\
                      &          &          &          &          & $(0.15)$ &          &          \\
Tr. X Land            &          &          &          &          & $-0.01$  &          &          \\
                      &          &          &          &          & $(0.18)$ &          &          \\
\hline
N             & $1218$   & $1218$   & $1174$   & $1218$   & $1218$   & $1099$   & $1060$   \\
\hline
\end{tabular}
\end{scriptsize}
\caption{Least squares regression estimates of 2015 sample intention-to-treat and covariate-interaction effects. Outcome is combined math-verbal test score, standardized. Standard errors account for village-level clustering.
 *Model 6 omits Tajik households.
 **Model 7 restrits to communities with same NGO as 2008}
\label{itt-interactions-2015}
\end{center}
\end{table}


==> ITT-interactions-2015.tex <==

\begin{table}
\begin{center}
\begin{scriptsize}
\begin{tabular}{l c c c c c c c}
\hline
 & 1 & 2 & 3 & 4 & 5 & 6* & 7** \\
\hline
Control mean          & $-0.19$  & $-0.18$  & $-0.20$  & $-0.18$  & $-0.18$  & $-0.21$  & $-0.19$  \\
                      & $(0.10)$ & $(0.12)$ & $(0.12)$ & $(0.12)$ & $(0.12)$ & $(0.13)$ & $(0.13)$ \\
Treatment             & $0.38$   & $0.36$   & $0.38$   & $0.35$   & $0.35$   & $0.38$   & $0.36$   \\
                      & $(0.11)$ & $(0.13)$ & $(0.13)$ & $(0.13)$ & $(0.13)$ & $(0.14)$ & $(0.15)$ \\
Child's age           & $0.26$   &          &          &          &          &          &          \\
                      & $(0.04)$ &          &          &          &          &          &          \\
Tr. X Child's age     & $0.00$   &          &          &          &          &          &          \\
                      & $(0.05)$ &          &          &          &          &          &          \\
HH. head age          &          & $0.00$   &          &          &          &          &          \\
                      &          & $(0.00)$ &          &          &          &          &          \\
Tr. X HH. head age    &          & $0.00$   &          &          &          &          &          \\
                      &          & $(0.00)$ &          &          &          &          &          \\
HH. head school       &          &          & $0.02$   &          &          &          &          \\
                      &          &          & $(0.01)$ &          &          &          &          \\
Tr. X HH. head school &          &          & $-0.00$  &          &          &          &          \\
                      &          &          & $(0.02)$ &          &          &          &          \\
HH. head farm.        &          &          &          & $-0.19$  &          &          &          \\
                      &          &          &          & $(0.11)$ &          &          &          \\
Tr. X HH. head farm.  &          &          &          & $0.07$   &          &          &          \\
                      &          &          &          & $(0.13)$ &          &          &          \\
Land                  &          &          &          &          & $-0.10$  &          &          \\
                      &          &          &          &          & $(0.15)$ &          &          \\
Tr. X Land            &          &          &          &          & $-0.01$  &          &          \\
                      &          &          &          &          & $(0.18)$ &          &          \\
\hline
R$^2$                 & $0.24$   & $0.06$   & $0.06$   & $0.06$   & $0.06$   & $0.06$   & $0.06$   \\
Adj. R$^2$            & $0.24$   & $0.05$   & $0.06$   & $0.06$   & $0.05$   & $0.06$   & $0.05$   \\
Num. obs.             & $1218$   & $1218$   & $1174$   & $1218$   & $1218$   & $1099$   & $1060$   \\
RMSE                  & $1.84$   & $2.05$   & $2.06$   & $2.05$   & $2.06$   & $2.02$   & $2.04$   \\
N Clusters            & $74$     & $74$     & $74$     & $74$     & $74$     & $65$     & $59$     \\
\hline
\end{tabular}
\end{scriptsize}
\caption{Least squares regression estimates of 2015 sample intention-to-treat and covariate-interaction effects. Outcome is combined math-verbal test score, standardized. Standard errors account for village-level clustering.
 *Model 6 omits Tajik households.
 **Model 7 restrits to communities with same NGO as 2008}
\label{itt-interactions-2015}
\end{center}
\end{table}


==> ITT_weighted.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Apr  7 14:58:20 2021
\begin{table}[!t]
\centering
\begin{tabular}{lrrr}
   \hline
 & t=1 (2008) unweighted & t=1 (2008) weighted & t=2 (2015) \\ 
   \hline
ITT Effect & 0.73 & 0.78 & 0.35 \\ 
    & (0.11) & (0.14) & (0.13) \\ 
  Control mean & -0.36 & -0.23 & -0.17 \\ 
    & (0.09) & (0.14) & (0.12) \\ 
   \hline
N & 689 & 689 & 1218 \\ 
   \hline
\end{tabular}
\caption{Least squares regression estimates of the intention-to-treat (ITT) effects and control group means. Outcome is combined math-verbal test score, standardized. Standard errors accounting for village-level clustering in parentheses.} 
\label{itt-table}
\end{table}


==> LATE_weighted.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Apr  7 14:58:59 2021
\begin{table}[!t]
\centering
\begin{tabular}{lrrr}
   \hline
 & t=1 (2008) unweighted & t=1 (2008) weighted & t=2 (2015) \\ 
   \hline
LATE & 1.06 & 1.06 & 1.04 \\ 
    & (0.14) & (0.22) & (0.53) \\ 
   \hline
First stage & 0.69 & 0.73 & 0.35 \\ 
    & (0.04) & (0.03) & (0.07) \\ 
   \hline
N & 1218 & N & 1218 \\ 
   \hline
\end{tabular}
\caption{Two-stage least squares regression estimates of the LATE on test scores, and least squares regression estimates of the first stage effect on CBE take-up. Standard errors accounting for village-level clustering in parentheses.} 
\label{late-table}
\end{table}


==> Xsum.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Apr  7 14:58:27 2021
\begin{table}[!t]
\centering
\begin{tabular}{llrrr}
   \hline
Covariate &  & t=1 (2008) & t=1 (2008, weighted) & t=2 (2015) \\ 
   \hline
Child's age (in yrs.) & mean & 8.58 & 8.71 & 8.26 \\ 
   & (sd) & (1.56) & (1.58) & (1.51) \\ 
   &  &  &  &  \\ 
  Household head age (in yrs.) & mean & 40.61 & 39.99 & 45.03 \\ 
   & (sd) & (10.57) & (10.43) & (15.67) \\ 
   &  &  &  &  \\ 
  Household head yrs. of school & mean & 3.35 & 3.75 & 2.93 \\ 
   & (sd) & (3.39) & (3.86) & (2.97) \\ 
   &  &  &  &  \\ 
  Household head farmer (0/1) & mean & 0.77 & 0.74 & 0.56 \\ 
   & (sd) & (0.42) & (0.44) & (0.50) \\ 
   &  &  &  &  \\ 
  Land owned (jeribs) & mean & 1.13 & 1.07 & 0.69 \\ 
   & (sd) & (1.50) & (1.44) & (0.46) \\ 
   &  &  &  &  \\ 
  Tajik ethnicity (0/1) & mean & 0.26 & 0.23 & 0.11 \\ 
   & (sd) & (0.44) & (0.42) & (0.32) \\ 
   &  &  &  &  \\ 
  NGO from 2008 (0/1) & mean & 1.00 & 1.00 & 0.87 \\ 
   & (sd) & (0.00) & (0.00) & (0.34) \\ 
   &  &  &  &  \\ 
   \hline
N &  & 689 & 689 & 1218 \\ 
   \hline
\end{tabular}
\caption{Covariates means and standard deviations (in parentheses) for the t=1 (in 2008, both unweighted and weighted) and t=2 (in 2015) study populations.} 
\label{xsum-table}
\end{table}


==> asymptotics.tex <==
Let's denote $\frac{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{e(X_{it})}\If(D_{it} = 2)\If(Y_{it} < c_{t,1})}{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{e(X_{it})}\If(D_{it} = 2)}$ as $\kappa_1$, $\frac{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})}\If(D_{it} = 0)Y_{it}}{\sum_{i=1}^{N_t} \frac{Z_{it}\If(D_{it} = 0)}{e(X_{it})}}$ as $\kappa_2$, and $\frac{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})}\If(D_{it} = 1)}{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})}}$ as $\kappa_3$ . We further denote parameters $\{\mu_t(-b_y, c_{t,1}; 1, 2), \mu_t(-b_y, c_{t,1}; 0, 2), \mu^0_t(0,2), c_{t,1}, \kappa_1, \kappa_2\}$ as $\theta$ and parameters $\{\pi_t(0,0), \pi_t(0,2), \pi_t(1,2), \pi_t(2,2), \kappa_3\}$ as $\gamma$. The parameter of interest, $\tau_t^L(0,2;(0,2))$, is equal to $\beta_{t,L}(0,2) - \mu^0_t(0,2) = \frac{\pi_t(0,2)+\pi_t(1,2)+ \pi_t(2,2)}{ \pi_t(0,2)}\mu_t(-b_y, c_{t,1}; 1, 2)  - \frac{\pi_t(2,2)}{\pi_t(0,2)} \mu_t(-b_y,  c_{t,1}; 0, 2) - \mu^0_t(0,2)$. The whole estimation process could be seen as a GMM estimator with the following moment conditions. For simplicity, we will ignore covariates.

\begin{align}
& Z_{it}\If(D_{it}=2)\left(\If (Y_{it} < c_{t,1})Y_{it} - \mu_t(-b_y, c_{t,1}; 1, 2)\right) \\
& (1-Z_{it})\If(D_{it}=2)\left(\If(Y_{it} < c_{t,1})Y_{it} - \mu_t(-b_y, c_{t,1}; 0, 2)\right) \\
& (1-Z_{it})\If(D_{it}=2)\left[\kappa_1 - \If(Y_{it} < c_{t,1})\right] \\
& Z_{it}\If(D_{it}=2)\left[\pi_t(2,2)\kappa_1 + \pi_t(0,2) - (\pi_t(0,2) + \pi_t(1,2) + \pi_t(2,2)) \If(Y_{it} < c_{t,1})\right] \\
& (1-Z_{it})\If(D_{it}=0)\left[(\pi_{t}(0,0) + \pi_{t}(0,2))Y_{it} - \pi_{t}(0,2)\mu^0_t(0,2) - \pi_{t}(0,0)\kappa_2 \right] \\ 
& Z_{it}\If(D_{it}=0)(Y_{it} - \kappa_2) \\
& Z_{it}\left[\pi_t(0,0) - \If(D_{it} = 0)\right] \\
& (1-Z_{it})\left[\pi_t(2,2) - \If(D_{it} = 2)\right] \\
& (1-Z_{it})\left[\pi_t(0,2) + \pi_t(0,0) - \If(D_{it} = 0)\right] \\
& (1-Z_{it})\left[\pi_t(1,2) + \kappa_3 - \If(D_{it} = 1)\right] \\
& Z_{it}\left[\kappa_3 - \If(D_{it} = 1)\right] 
\end{align}
Let $\mathbf{h} (w;\theta, \gamma) = (\mathbf{g} (w;\theta, \gamma), \mathbf{m} (w; \gamma))$ be the moment conditions above. We will rely on results in \citet{newey1994large} to show that the estimates are consistent and normally distributed as $N \rightarrow \infty$. 

For consistency, we apply Theorem 2.6 in \citet{newey1994large} to our $\mathbf{h} (w;\theta, \gamma)$. It is easy to easy that the equations lead to a unique solution. As long as $Y_{it}$ is bounded, we know that all the parameters, nuisance or not, are within a compact set. Hence, condition (ii) is satisfied. Condition (iii), the continuity of $\mathbf{h} (w;\theta, \gamma)$ is obvious and condition (iv) will follow.

Theorem 7.2 in \citet{newey1994large} is needed to show the asymptotic normality of the estimates. Condition (i) and (iii) are satisfied due to the same reason stated above. (iv) holds due to the central limit theorem. (ii) could be verified using matrix $\mathbf{H}$ described below. We use Theorem 1 in \citet{andrews1994asymptotics} to show the stochastic equicontinuity of $\mathbf{h} (w;\theta, \gamma)$. Assumption C is obvious. The envelop function is constructed following the example in \citet{lee2009training}. For moments (3) (4) (7)-(12), the envelop is set to be 3. For moments (1) and (2), the envelop is $|Y_{it} - \mu_{t0}| + \sup_{\mu_{t}} |\mu_{t0} - \mu_{t}|$ where $\mu_{t}$ is the corresponding parameter and $\mu_{t0}$ is its true value. For moment (5), the envelop is $|Y_{it}| + 1$. Then assumption A is satisfied. Assumption B holds as the outcome $Y_{it}$ is bounded.

Notice that $\mathbf{h}_0(w;\theta, \gamma) = \E\left[\mathbf{h} (w;\theta, \gamma)\right]$ equals to:
\begin{align*}
& P(D_{it}=2,  Z_{it}=1)\left( \int_{-b_y}^{c_{t,1}} y_{it} f_{Y_{it}|Z_{it=1}, D_{it}=2}(y_{it})d y_{it} - \mu_t(-b_y, c_{t,1}; 1, 2)\right) \\
& P(D_{it}=2, Z_{it}=0) \left(\int_{-b_y}^{c_{t,1}} y_{it} f_{Y_{it}|Z_{it=0}, D_{it}=2}(y_{it}) d y_{it} - \mu_t(-b_y, c_{t,1}; 0, 2)\right) \\
& P(D_{it}=2, Z_{it}=0)\left[\kappa_1 - F_{Y_{it} | D_{it}=2, Z_{it}=0}(c_{t,1})\right]   \\
& P(D_{it}=2, Z_{it}=1)\left[\pi_t(2,2)\kappa_1 + \pi_t(0,2) -  (\pi_t(0,2) + \pi_t(1,2) + \pi_t(2,2)) F_{Y_{it} | D_{it}=2, Z_{it}=1}(c_{t,1})\right]   \\
& P(D_{it}=0, Z_{it}=0)\left[(\pi_{t}(0,0) + \pi_{t}(0,2))\E(Y_{it}|D_{it}=0, Z_{it}=0) - \pi_{t}(0,2)\mu^0_t(0,2) - \pi_{t}(0,0)\kappa_2 \right] \\ 
& P(D_{it}=0, Z_{it}=1)\left[\E(Y_{it}|D_{it}=0, Z_{it}=1) - \kappa_2\right] \\
& P(Z_{it}=1)\left[\pi_t(0,0) - P(D_{it} = 0 | Z_{it}=1)\right] \\
& P(Z_{it}=0)\left[\pi_t(2,2) - P(D_{it} = 2 | Z_{it}=0)\right] \\
& P(Z_{it}=0)\left[\pi_t(0,2) + \pi_t(2,2) - P(D_{it} = 0 | Z_{it}=0)\right] \\
& P(Z_{it}=0)\left[\pi_t(1,2) + \kappa_3 - P(D_{it} = 1 | Z_{it}=0)\right] \\
& P(Z_{it}=1)\left[\kappa_3 - P(D_{it} = 1 | Z_{it}=1)\right] 
\end{align*}
We know that $\mathbf{h}_0(w;\theta_0, \gamma_0) = 0$, where $(\theta_0, \gamma_0)$ are the true values of $(\theta, \gamma)$. Define $\mathbf{H}$ as $\frac{d \mathbf{h}_0}{d (\theta, \gamma)'}|_{(\theta_0, \gamma_0)} = \begin{pmatrix}
\mathbf{G}_{\theta_0} & \mathbf{G}_{\gamma_0} \\
\mathbf{0} & \mathbf{M}_{\gamma_0}
\end{pmatrix}$. $\mathbf{H}$ is a $11 \times 11$ matrix. Similarly, define $\mathbf{\Sigma}$ as $\E \left[\mathbf{h} (w;\theta, \gamma) \mathbf{h}' (w;\theta, \gamma) \right]|_{(\theta_0, \gamma_0)} = \begin{pmatrix}
\mathbf{\Sigma}_{11} & \mathbf{\Sigma}_{12} \\
\mathbf{\Sigma}_{21} & \mathbf{\Sigma}_{22}
\end{pmatrix}$. Then, \citet{andrews1994asymptotics} indicates that the asymptotic variance is $\mathbf{V} = \mathbf{H}^{-1}\mathbf{\Sigma} (\mathbf{H}^{'})^{-1}$. As $\sqrt{N}\begin{pmatrix}
\hat \theta \\
\hat \gamma \\
\end{pmatrix} - \begin{pmatrix}
\theta_0 \\
\gamma_0
\end{pmatrix} \rightarrow N(0, \mathbf{V})$, it is easy to see that $\tau_t^L(0,2;(0,2))$ is also normally distributed whose variance can be caluclated via the delta method.

To derive the analytical variance, we treat the estimation as a two-step process. In the first step, all the $\pi$s are estimated. In the second step, the estimates are ``plugged in" and treated as known. Now the first six moments are used to estimate the parameters in the second step, and the last five moments are for the first-step parameters. To save space, we ignore the time index and write $\mu_t(-b_y, c_{t,1}; 1, 2)$ as $\mu_{12}$,  $\mu_t(-b_y, c_{t,1}; 0, 2)$ as $\mu_{02}$, $\mu^0_t(0,2)$ as $\mu^0$, $P(D_{it}=d)$ as $P_{Dd}$, $P(Z_{it}=z)$ as $P_{Zz}$, $P(D_{it}=d, Z_{it}=z)$ as $P_{DdZz}$, $F_{Y_{it}|Z_{it}=z, D_{it}=d}(c_{t,1})$ as $F_{dz}(c_1)$, $f_{Y_{it}|Z_{it}=z, D_{it}=d}(c_{t,1})$ as $f_{dz}(c_{1})$.

 Now the variance-covariance matrix for $\theta$ at $\theta_0$ is:
\begin{align*}
\mathbf{V}_{\theta_0} = \mathbf{G}_{\theta_0}^{-1}\E\left[\left(\mathbf{g} (w;\theta_0, \gamma_0)- \mathbf{G}_{\gamma_0}\mathbf{M}_{\gamma_0}^{-1}\mathbf{m} (w; \gamma_0)\right) \left(\mathbf{g} (w;\theta_0, \gamma_0)- \mathbf{G}_{\gamma_0}\mathbf{M}_{\gamma_0}^{-1}\mathbf{m} (w; \gamma_0) \right)^{'} \right] (\mathbf{G}_{\theta_0}^{'})^{-1}
\end{align*} 
It is easy to see:
\begin{align*}
\mathbf{G}_{\theta_0} = (\mathbf{G}_{1\theta_0}, \mathbf{G}_{2\theta_0})
\end{align*}
where

\begin{align*}
\mathbf{G}_{1\theta_0} = \begin{pmatrix}
-P_{D2Z1} & 0 & 0  \\
0 & -P_{D2Z0} & 0  \\
0 & 0 & 0  \\
0 & 0 & 0  \\
0 & 0 & -P_{D0Z0}\pi(0,2) \\
0 & 0 & 0 \\
\end{pmatrix}
\end{align*}
and

\begin{align*}
\mathbf{G}_{2\theta_0} = \begin{pmatrix}
P_{D2Z1}c_{1}f_{21}(c_{1}) & 0 & 0 \\
P_{D2Z0}c_{1} f_{20}(c_{1})  & 0 & 0 \\
-P_{D2Z0}f_{20}(c_{1}) & P_{D2Z0} & 0 \\
 -P_{D2Z1} (\pi(0,2) + \pi(1,2) + \pi(2,2))f_{21}(c_{1}) & P_{D2Z1}\pi(2,2) & 0 \\
0 & 0 & -P_{D0Z0}\pi(0,0) \\
0 & 0 & -P_{D0Z1} \\
\end{pmatrix}
\end{align*}

Let $a_1 = - (\pi(0,2) + \pi(1,2) + \pi(2,2))f_{21}(c_{t,1}) + \pi(2,2)f_{20}(c_{1})$, then we can write the inverse of $G_{\theta_0}$ as:
\begin{align*}
&\mathbf{G}_{\theta_0}^{-1} = (\mathbf{G}_{1\theta_0}^{-1}, \mathbf{G}_{2\theta_0}^{-1})
\end{align*}
where

\begin{align*}
\mathbf{G}_{1\theta_0}^{-1} = \begin{pmatrix}
\frac{1}{-P_{D2Z1}} & 0 & -\frac{\pi(2,2)c_{1} f_{21}(c_{1})}{a_1 P_{D2Z0}} \\
0 & -\frac{1}{P_{D2Z0}} & -\frac{\pi(2,2)c_{1} f_{20}(c_{1})}{a_1 P_{D2Z0}}  \\
0 & 0 & 0  \\
0 & 0 & -\frac{\pi(2,2)}{a_1 P_{D2Z0}} \\
0 & 0 & \frac{1}{P_{D2Z0}} - \frac{\pi(2,2)f_{20}(c_{t,1})}{a_1 P_{D2Z0}}  \\
0 & 0 & 0 
\end{pmatrix}
\end{align*}
and

\begin{align*}
\mathbf{G}_{2\theta_0}^{-1} = \begin{pmatrix}
\frac{c_{1} f_{21}(c_{1})}{a_1 P_{D2Z1}} & 0 & 0 \\
\frac{c_{1} f_{20}(c_{1})}{a_1 P_{D2Z1}} & 0 & 0  \\
0 & -\frac{1}{P_{D0Z0}\pi(0,2)} & \frac{\pi(0,0)}{P_{D0Z1}\pi(0,2)}  \\
\frac{1}{a_1 P_{D2Z1}} & 0 & 0  \\
\frac{f_{20}(c_{1})}{a_1 P_{D2Z1}} & 0 & 0 \\
0 & 0 & -\frac{1}{P_{D0Z1}}  \\
\end{pmatrix}
\end{align*}
Similarly, $\mathbf{\Sigma}_{11} = \E \left[\mathbf{g} (w;\theta_0, \gamma_0) \mathbf{g}' (w;\theta_0, \gamma_0) \right] = (\mathbf{\Sigma}_{11,1}, \mathbf{\Sigma}_{11,2})$. Let $a_2 = \pi(2,2)\kappa_1 + \pi(0,2)$, $a_3 = \pi(0,2) + \pi(1,2) + \pi(2,2)$, $a_4 = \pi(0, 0) + \pi(0, 2)$, $a_5 = \pi(0,2)\mu^0 + \pi(0,0)\kappa_2$, $\E_{dz}\left[Y_i^k\right] = \E\left[Y_i^k | D_i = d, Z_i = z \right]$, and $\Var_{dz}\left[Y_i^k\right] = \Var\left[Y_i^k | D_i = d, Z_i = z \right]$, then:
\begin{scriptsize}
\begin{align*}
& \mathbf{\Sigma}_{11,1} = \\
& \begin{pmatrix}
P_{D2Z1}\left( \int_{-b_y}^{c_{1}} y_{i}^2  f_{21}(y_{i})d y_{i}- \mu_{12}^2\right) & 0 & 0 \\
0 & P_{D2Z0}\left(\int_{-b_y}^{c_{1}} y_{t}^2 f_{20}(y_{i})d y_{i}- \mu_{02}^2\right) & (\kappa_1 - 1) P_{D2Z0}\left( \int_{-b_y}^{c_{1}} y_{i} f_{20}(y_{i})d y_{i} - \mu_{02}\right) \\
0 & (\kappa_1 - 1) P_{D2Z0}\left(\int_{-b_y}^{c_{1}} y_{i} f_{20}(y_{i})d y_{i} - \mu_{02}\right) & P_{D2Z0}(\kappa_1 -  F_{20}(c_1))^{2}  \\
(a_2 - a_3) P_{D2Z1} \left(\int_{-b_y}^{c_{1}} y_{i} f_{21}(y_{i})d y_{i} - \mu_{12}\right) & 0 & 0  \\
0 & 0 & 0 \\
0 & 0 & 0  \\
\end{pmatrix}
\end{align*}
\end{scriptsize}
and
\begin{scriptsize}
\begin{align*}
& \mathbf{\Sigma}_{11,2} = \\
& \begin{pmatrix}
(a_2 - a_3) P_{D2Z1}\left(\int_{-b_y}^{c_{1}} y_{i} f_{21}(y_{i})d y_{i} - \mu_{12}\right) & 0 & 0 \\
0 & 0 & 0 \\
0 & 0 & 0  \\
P_{D2Z1}(a_2^2 - 2 a_2 a_3F_{21}(c_1) + a_3^2 F_{21}(c_1))  & 0 & 0  \\
0 & P_{D0Z0}\E_{00}\left[a_4 Y_i - a_5 \right]^2 & 0 \\
0 & 0  & P_{D0Z1}\E_{01}\left[Y_i - \kappa_4\right]^2  \\
\end{pmatrix}
\end{align*}
\end{scriptsize}
Exploiting the fact that moment conditions as well as the fact that their expectations equal to zero, we have:
\begin{scriptsize}
\begin{align*}
& \mathbf{\Sigma}_{11,1} = \\
& \begin{pmatrix}
P_{D2Z1}\left( \int_{-b_y}^{c_{1}} y_{i}^2  f_{21}(y_{i})d y_{i}- \mu_{12}^2\right) & 0 & 0 \\
0 & P_{D2Z0}\left(\int_{-b_y}^{c_{1}} y_{t}^2 f_{20}(y_{i})d y_{i}- \mu_{02}^2\right) & 0 \\
0 & 0 & P_{D2Z0}\kappa_1(1-\kappa_1)  \\
0 & 0 & 0  \\
0 & 0 & 0  \\
0 & 0 & 0 
\end{pmatrix}
\end{align*}
\end{scriptsize}
and
\begin{scriptsize}
\begin{align*}
& \mathbf{\Sigma}_{11,2} = \\
& \begin{pmatrix}
0 & 0 & 0  \\
0 & 0 & 0  \\
0 & 0 & 0  \\
P_{D2Z1}a_2 (a_3 - a_2) & 0 & 0 \\
0 & P_{D0Z0}a_4^2 \Var_{00}\left[Y_i \right] & 0 \\
0 & 0 & P_{D0Z1}\Var_{01}\left[Y_i \right]
\end{pmatrix}
\end{align*}
\end{scriptsize}
Now, $\mathbf{\tilde{V}}_{\theta_0} = \mathbf{G}_{\theta_0}^{-1}\mathbf{\Sigma}_{11} (\mathbf{G}_{\theta_0}^{'})^{-1}$ is the variance of $\theta$ at $\theta_0$
if we ignore the uncertainty induced by the first stage. In this case, we have:

\begin{align*}
& \Var(\mu_t(-b_y, c_{t,1}; 1, 2)) = \frac{\int_{-b_y}^{c_{1}} y_{i}^2 f_{21}(y_{i})d y_{i}  - \mu_{12}^2}{P_{D2Z1}} \\
& \Var(\mu_t(-b_y, c_{t,1}; 0, 2)) = \frac{\int_{-b_y}^{c_{1}} y_{i}^2 f_{20}(y_{i})d y_{i}  - \mu_{02}^2}{P_{D2Z0}} \\
& \Cov(\mu_t(-b_y, c_{t,1}; 1, 2), \mu_t(-b_y, c_{t,1}; 0, 2)) = 0
\end{align*}
and
\begin{align*}
\Var( \mu^0_t(0,2)) = & \frac{(\pi(0,0) + \pi(0,2))^2}{P_{D0Z0}\pi^2(0,2)} \Var_{00}\left[Y_i\right] \\
& + \frac{\pi^2(0,0)}{P_{D0Z1}\pi^2(0,2)} \Var_{01}\left[Y_i\right] \\
\end{align*}
\begin{align*}
& \Cov(\mu_t(-b_y, c_{t,1}; 1, 2), \mu^0_t(0,2)) = 0 \\
& \Cov(\mu_t(-b_y, c_{t,1}; 0, 2), \mu^0_t(0,2)) = 0
\end{align*}

To proceed, we have:
\begin{footnotesize}
\begin{align*}
& \mathbf{G}_{\gamma} = \\
& \begin{pmatrix}
0 & 0 & 0 & 0 & 0  \\
0 & 0 & 0  & 0 & 0  \\
0 & 0 & 0  & 0 & 0  \\
0 & P_{D2Z1}(1-F_{21}(c_1)) & -P_{D2Z1}F_{21}(c_1) & P_{D2Z1}\left(\kappa_1 - F_{21}(c_1) \right) & 0 \\
P_{D0Z0}(\E_{00}Y_i - \kappa_4) & P_{D0Z0}(\E_{00}Y_i - \mu^0) & 0 & 0 & 0 \\
0 & 0 & 0  & 0 & 0 \\
\end{pmatrix}
\end{align*}
\end{footnotesize}

\begin{align*}
\mathbf{M}_{\gamma} = \begin{pmatrix}
P_{Z1}& 0 & 0 & 0 & 0 \\
0 & 0 & 0  & P_{Z0} & 0 \\
0 & P_{Z0} & 0 & P_{Z0} & 0 \\
0 & 0 & P_{Z0} & 0 & P_{Z0} \\
0 & 0 & 0 & 0 & P_{Z1}
\end{pmatrix}
\end{align*}
and

\begin{scriptsize}
\begin{align*}
& \mathbf{\Sigma}_{22} = \E\left[\mathbf{m} (w; \gamma) \mathbf{m}^{'} (w; \gamma)\right] \\
& = \begin{pmatrix}
P_{Z1}(\pi_{00} - \pi_{00}^2) & 0 & 0 & 0 & -P_{Z1}\kappa_3 \pi_{00} \\
0 & P_{Z0}(\pi_{22} - \pi_{22}^2) & -P_{Z0}\pi_{22}(\pi_{00} + \pi_{02}) & -P_{Z0}\pi_{22}(\pi_{12}+\kappa_3) & 0  \\
0 & -P_{Z0}\pi_{22}(\pi_{00} + \pi_{02}) & P_{Z0}(p_{00} - p_{00}^2) & -P_{Z0}\pi_{12}(\pi_{00} + \pi_{02}) & 0 \\
0 & -P_{Z0}\pi_{22}(\pi_{12}+\kappa_3) & -P_{Z0}\pi_{12}(\pi_{00} + \pi_{02}) & P_{Z0}(p_{10} - p_{10}^2) & 0 \\
-P_{Z1}\kappa_3 \pi_{00} & 0 & 0 &  0 & P_{Z1}(p_{11} - p_{11}^2) 
\end{pmatrix}
\end{align*}
\end{scriptsize}
We also know that $\mathbf{\Sigma}_{12} = \mathbf{\Sigma}_{21} = \mathbf{0}$. Then the variance-covariance matrix $\mathbf{V}$ can be calculated as $\mathbf{H}^{-1}\mathbf{\Sigma} (\mathbf{H}^{'})^{-1}$.

Finally, as $\tau_t^L(0,2;(0,2)) = f(\mu_t(-b_y, c_{t,1}; 1, 2), \mu_t(-b_y, c_{t,1}; 0, 2), \mu^0_t(0,2), \pi_t(0,2), \pi_t(1,2), \pi_t(2,2)) = f(\eta)$, we can use the delta method to derive the asymptotic distribution of $\tau_t^L(0,2;(0,2))$:
\begin{align*}
\Var(\tau_t^L(0,2;(0,2))) = (\frac{d f}{d \eta})^{'} \mathbf{V}_{\eta} \frac{d f}{d \eta}
\end{align*}
where $\frac{d f}{d \eta} = (\frac{\pi_{02} + \pi_{12} + \pi_{22}}{\pi_{02}}, -\frac{\pi_{22}}{\pi_{02}}, -1, -\frac{\pi_{12} + \pi_{22}}{\pi_{02}^2}\mu_{12} +\frac{\pi_{22}}{\pi^2_{02}}\mu_{02}, \frac{1}{\pi_{02}}\mu_{12}, \frac{1}{\pi_{02}}(\mu_{12} - \mu_{02}))^{'}$,
and $\mathbf{V}_{\eta}$ is the corresponding submatrix of $\mathbf{V}$. The variances of $\tau_t^U(0,2;(0,2))$, $\tau_t^L(1,2;(1,2))$, and $\tau_t^U(1,2;(1,2))$ can be similarly obtained.





==> attendance.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Apr  7 14:58:49 2021
\begin{table}[!t]
\centering
\begin{tabular}{|l|rr|rr|}
  \hline
  & \multicolumn{2}{c|}{2008 } &  \multicolumn{2}{c|}{2015} \\
 \hline
 & Control & Treated & Control & Treated \\ 
   \hline
No school & 0.66 & 0.23 & 0.36 & 0.20 \\ 
  Govt. school & 0.34 & 0.09 & 0.45 & 0.25 \\ 
  CBE & 0.00 & 0.67 & 0.18 & 0.54 \\ 
   \hline
\end{tabular}
\caption{Attendance rates for girls in control (no CBE) and treated (with CBE) communities in the t=1 (in 2008, estimated using balancing weights) and t=2 (in 2015) study populations.} 
\label{attendance}
\end{table}


==> bounds.tex <==
Let's denote the complier average causal effect, $\E \left[Y_{it}(2) -  Y_{it}(0) | S_{it} = (0,2) \right]$, as $\tau_t(0,2;(0,2))$, and the substitutor causal effect, $\E\left[Y_{it}(2) - Y_{it}(1) | S_{it} = (1,2) \right]$, as $\tau_t(1,2;(1,2))$, then
\begin{prop}\label{prop:bounds}
Suppose Assumptions \ref{assn:monotonicity}-\ref{assn:cia} hold and $Y_{it}(d)$ is continuous for all $d \in \mathcal{D}$. Then,
\begin{enumerate}[(i)]
\item $$
\beta_{t,L}(0,2) \le E\left[Y_{it}(2)|S_{it}=(0,2)\right] \le \beta_{t,U}(0,2),
$$ 
where
\begin{align*}
\beta_{t,L}(0,2) = & \frac{\pi_t(0,2)+\pi_t(1,2)}{\pi_t(0,2)}  \int_{-b_y}^{c_{t,1}} y d \tilde{F}_{t,Y_{it}(2)}(y)
\end{align*}
and
\begin{align*}
\beta_{t,U}(0,2) = & \frac{\pi_t(0,2)+\pi_t(1,2)}{\pi_t(0,2)}  \int^{b_y}_{c_{t,2}} y d \tilde{F}_{t,Y_{it}(2)}(y),
\end{align*}
with 
\begin{align*}
\tilde{F}_{t,Y_{it}(2)}(y) %& \equiv  F_{t,Y_{it}(2)}(y|S_{it} \in \{(0,2),(1,2) \})\\
&=  \frac{\pi_t(0,2)+\pi_t(1,2) +\pi_t(2,2)}{\pi_t(0,2)+\pi_t(1,2)}F_{t,Y_{it}(2)}(y|Z_{it}=1, D_{it}=2) \\
& \hspace{2em} - \frac{\pi_t(2,2)}{\pi_t(0,2)+\pi_t(1,2)}F_{t,Y_{it}(2)}(y|Z_{it}=0, D_{it}=2),\\
%\pi_t(\cdot,2) & \equiv \pi_t(0,2)+\pi_t(1,2) +\pi_t(2,2) = \Pr[D_{it}(1)=2], \text{ and}\\
c_{t,1} & \equiv \tilde{F}_{t,Y_{it}(2)}^{-1}\left(\frac{\pi_t(0,2)}{\pi_t(0,2)+\pi_t(1,2)} \right), \text{ and}\\
c_{t,2} & \equiv \tilde{F}_{t,Y_{it}(2)}^{-1}\left(\frac{\pi_t(1,2)}{\pi_t(0,2)+\pi_t(1,2)} \right).
\end{align*}
where $F_{t,V(v)}$ is the distribution function in context $t$ for a random variable $V$ and $F_{t,V}^{-1}(r)$ gives the quantile at point $r$ in the distribution function.
\item The bounds $[\beta_{t,L}(0,2), \beta_{t,U}(0,2)]$ are sharp for $E\left[Y_{it}(2)|S=(0,2)\right]$ with respect to the mixture distribution, $F_{t,Y_{it}(2)}\left(y|S_{it} \in \{(0,2), (1,2)\}\right)$.
\item 
$$
\beta_{t,L}(0,2) - \mu^0_t(0,2) \le \tau_t(0,2;(0,2)) \le \beta_{t,U}(0,2) - \mu^0_t(0,2).
$$
\end{enumerate}
\end{prop}

\noindent{\it Proof.} We cannot disentangle the distribution of $Y_{it}(2)$ outcomes for $S_{it} = (0,2)$ and $S_{it} = (1,2)$ types. Rather, these distributions are combined in the mixture distribution,
\begin{align}
F_{t,Y_{it}(2)}\left(y|S_{it} \in \{(0,2), (1,2)\}\right) = & \frac{\pi_t(0,2)}{\pi_t(0,2)+\pi_t(1,2)}F_{t,Y_{it}(2)}\left(y|S_{it} = (0,2)\right) \nonumber\\
&  + \frac{\pi_t(1,2)}{\pi_t(0,2)+\pi_t(1,2)}F_{t,Y_{it}(2)}\left(y|S_{it}=(1,2) \right).\label{eq:mix}
\end{align}
Under the assumptions, the mixture distribution is identified  by the data as,
\begin{align*}
F_{t,Y_{it}(2)}\left(y|S_{it} \in \{(0,2), (1,2)\}\right) & =  \frac{\pi_t(0, 2)+\pi_t(1, 2)+\pi_t(2, 2)}{\pi_t(0,2)+\pi_t(1,2)}F_{t,Y_{it}(2)}(y|S_{it} \in \{(0,2),(1,2),(2,2)\}) \\
& \hspace{1em} - \frac{\pi_t(2,2)}{\pi_t(0,2)+\pi_t(1,2)}F_{t,Y_{it}(2)}(y|S_{it} = (2,2)) \\
& =  \frac{\pi_t(\cdot, 2)}{\pi_t(0,2)+\pi_t(1,2)}F_{t,Y_{it}(2)}(y|Z_{it}=1, D_{it}=2) \\
& \hspace{1em} - \frac{\pi_t(2,2)}{\pi_t(0,2)+\pi_t(1,2)}F_{t,Y_{it}(2)}(y|Z_{it}=0, D_{it}=2)\\
& = \tilde F_{t,Y_{it}(2)}(y).
\end{align*}
Now consider $\beta_{t,L}(0,2)$ as defined above.  As is clear from expression \eqref{eq:mix}, no subpopulation with proportion $\frac{\pi_t(0,2)}{\pi_t(0,2)+\pi_t(1,2)}$ from the population distributed as $F_{t,Y_{it}(2)}\left(y|S_{it} \in \{(0,2), (1,2)\}\right)$ could have a mean smaller than $\beta_{t,L}(0,2)$, given that $\beta_{t,L}(0,2)$ concentrates all values into the bottom left of the distribution. This establishes $\beta_{t,L}(0,2) \le E\left[Y_{it}(2)|S=(0,2)\right]$, and a similar argument establishes $ \beta_{t,U}(0,2) \ge E\left[Y_{it}(2)|S=(0,2)\right]$, proving (i). For (ii), sharpness of the bounds follows from \citet[Corollary 4.1]{horowitz1995identification} as applied to expression \eqref{eq:mix} and the fact that the cut point, $c_{t}$, is uniquely determined by continuity of $Y_{it}(2)$ and the uniqueness of $\frac{\pi_t(0,2)}{\pi_t(0,2)+\pi_t(1,2)}$ . Then (iii) follows from the expressions for $\mu_t^0(0,2)$ and $\tau_t(0,2;(0,2))$.\hspace{1em}$\square$

We have similar results for $\tau_t(1,2;(1,2))$, which are omitted to save space.


==> bounds_boot.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Apr  7 15:52:06 2021
\begin{table}[!t]
\centering
\begin{tabular}{lrrrr}
   \hline
Year & 2008 & 2008 & 2015 & 2015 \\ 
 & Lower bound, t=1 & Upper bound, t=1 & Lower bound, t=2 & Upper bound, t=2 \\ 
   \hline
  Compliers & 0.54 & 1.77 & 0.99 & 2.08 \\ 
  & (0.24,0.83) & (1.46,2.09) & (0.52,1.46) & (1.60,2.56) \\ 
 \hline
  Substitutors & -0.03 & 2.08 & 0.17 & 1.02 \\ 
  & (-0.65,0.59) & (1.30,2.86) & (-0.29,0.62) & (0.61,1.44) \\ 
   \hline
\end{tabular}
\caption{Bound estimates of the effect on compliers and substitutors. Bootstrap 95\% confidence interval in parentheses.} 
\label{bounds_boot-table}
\end{table}


==> estimators.tex <==
In this section, we present estimators for each parameter of interest mentioned in the main text. First, let's define $p(d, z) = P(D_{it} = d, Z_{it} = z)$. Then, we estimate the share of each principal strata as follows:
\begin{align*}
& \hat \pi_t(1,2) = \hat p_t(1,0) - \hat p_t(1,1) \\
= & \frac{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{1-e(X_{it})}\If(D_{it} = 1)}{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{1-e(X_{it})}} - \frac{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})}\If(D_{it} = 1)}{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})}} \\
& \hat \pi_t(2,2) = \hat p_t(2,0) = \frac{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{1-e(X_{it})}\If(D_{it} = 2)}{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{1-e(X_{it})}} \\
& \hat \pi_t(0,0) = \hat p_t(0,1) = \frac{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})}\If(D_{it} = 0)}{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})}} \\
& \hat \pi_t(0,2) = \hat p_t(0,0) - \hat p_t(0,1) \\
= & \frac{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{1-e(X_{it})}\If(D_{it} = 0)}{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{1-e(X_{it})}} - \frac{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})}\If(D_{it} = 0)}{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})}}
\end{align*}

Next, for the intention to treat effect (ITT) and local average treatment effect (LATE), we have
\begin{align*}
\widehat{\text{ITT}}_t \equiv \frac{\sum_{i=1}^{N_t} Y_{it} \frac{Z_{it}}{e(X_{it})}}{\sum_{i=1}^{N_t}\frac{Z_{it}}{e(X_{it})}} - \frac{\sum_{i=1}^{N_t} Y_{it} \frac{1-Z_{it}}{1-e(X_{it})}}{\sum_{i=1}^{N_t}\frac{1-Z_{it}}{1-e(X_{it})}},
\end{align*}

\begin{align*}
\widehat{\text{LATE}}_t \equiv \frac{\widehat{\text{ITT}}_t }{\hat \pi_t(0,2)+\hat \pi_t(1,2)}.
\end{align*}

Then,  for the lower bound of $E\left[Y_{it}(2)|S_{it}=(0,2)\right]$, $\beta_{t,L}(0,2)$, defined in the previous section, we estimate it as follows:
\begin{align*}
\hat \beta_{t,L}(0,2) \equiv \frac{\hat \pi_t(0,2)+\hat \pi_t(1,2)}{\hat  \pi_t(0,2)} \left[ \hat \pi_{t1}\hat \mu_t(-b_y,\hat c_{t,1}; 1, 2)  -  \hat \pi_{t2}\hat \mu_t(-b_y, \hat c_{t,1}; 0, 2) \right]
\end{align*}
where $\hat \pi_{t1} = \frac{\hat \pi_t(0,2)+\hat \pi_t(1,2)+\hat \pi_t(2,2)}{\hat \pi_t(0,2)+\hat \pi_t(1,2)}$, $\hat \pi_{t2} = \frac{\hat \pi_t(2,2)}{\hat \pi_t(0,2)+\hat \pi_t(1,2)}$, and
$$
\hat \mu_t(u,v; z, d) \equiv \frac{\sum_{i=1}^{N_t} \left[z\frac{Z_{it}}{e(X_{it})} + (1-z)\frac{1-Z_{it}}{1-e(X_{it})}\right]\If(D_{it} = d)\If(u < Y_{it} < v)Y_{it} }{\sum_{i=1}^{N_t} \left[z\frac{Z_{it}}{e(X_{it})} + (1-z)\frac{1-Z_{it}}{1-e(X_{it})}\right]\If(D_{it} = d)}.
$$
In addition, $\hat c_{t,1}$ satisfies:
\begin{align*}
\tilde{F}_{t,Y_{it}(2)}(\hat c_{t,1}) = \frac{\hat \pi_t(0,2)}{\hat \pi_t(0,2)+ \hat \pi_t(1,2)} 
\end{align*}
where
\begin{align*}
\tilde{F}_{t,Y_{it}(2)}(\hat c_{t,1}) = & \frac{\hat \pi_t(0,2)+ \hat \pi_t(1,2) + \hat \pi_t(2,2)}{\hat \pi_t(0,2)+\hat \pi_t(1,2)}\hat F_{t,Y_{it}(2)}(\hat c_{t,1}|Z_{it}=1, D_{it}=2) \\
& -  \frac{\hat \pi_t(2,2)}{\hat \pi_t(0,2)+\hat \pi_t(1,2)}\hat F_{t,Y_{it}(2)}(\hat c_{t,1}|Z_{it}=0, D_{it}=2) \\
= & \frac{\hat \pi_t(0,2)+ \hat \pi_t(1,2) + \hat \pi_t(2,2)}{\hat \pi_t(0,2)+\hat \pi_t(1,2)}\frac{\sum_{i=1}^{N_t} \left[\frac{Z_{it}}{e(X_{it})}\right]\If(D_{it} = 2)\If(Y_{it} < \hat c_{t,1} )}{\sum_{i=1}^{N_t} \left[\frac{Z_{it}}{e(X_{it})} \right]\If(D_{it} = 2)} \\
& -  \frac{\hat \pi_t(2,2)}{\hat \pi_t(0,2)+\hat \pi_t(1,2)}\frac{\sum_{i=1}^{N_t} \left[\frac{1-Z_{it}}{1-e(X_{it})}\right]\If(D_{it} = 2)\If(Y_{it} < \hat c_{t,1} )}{\sum_{i=1}^{N_t} \left[\frac{1-Z_{it}}{1-e(X_{it})}\right]\If(D_{it} = 2)} \\
\end{align*}
The upper bound $\beta_{t,U}(0,2)$ can be similarly estimated and we omit the details to save space.

The conditional expectation $\mu^0_t(0,2)$ can be estimated via the following equation:

\begin{align*}
\hat \mu^0_t(0,2) = & \frac{\hat \pi_t(0,0)+\hat \pi_t(0,2)}{\hat \pi_t(0,2)}\frac{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{1-e(X_{it})}\If(D_{it}=0)Y_{it}}{\sum_{i=1}^{N_t} \frac{1-Z_{it}}{1-e(X_{it})}\If(D_{it}=0)}\\
& -\frac{\hat \pi_t(0,0)}{\hat \pi_t(0,2)}\frac{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})} \If(D_{it}=0)Y_{it}}{\sum_{i=1}^{N_t} \frac{Z_{it}}{e(X_{it})} \If(D_{it}=0)}.
\end{align*}

Finally, we estimate the lower bound of the complier average causal effect, $\tau_t^L(0,2;(0,2))$, via $\hat \beta_{t,L}(0,2) - \hat \mu^0_t(0,2)$. Similarly, we can estimate the upper bound of $\tau_t(0,2;(0,2))$, as well as the bounds for the substitutor causal effect, $\tau_t(1,2;(1,2))$.




==> strata-weighted.tex <==
% latex table generated in R 4.0.2 by xtable 1.8-4 package
% Wed Apr  7 14:59:06 2021
\begin{table}[!t]
\centering
\begin{tabular}{lrr}
   \hline
Principal stratum & t=1 & t=2 \\ 
   \hline
Never taker & 0.23 & 0.20 \\ 
  Govt. adherent & 0.09 & 0.25 \\ 
  Always taker & 0.00 & 0.18 \\ 
  Complier & 0.42 & 0.16 \\ 
  Substitutor & 0.25 & 0.20 \\ 
   \hline
\end{tabular}
\caption{Weighted estimation distribution of girls population across principal strata in the t=1 (in 2008) and t=2 (in 2015) study populations, assuming monotonicity.  Shares may not add up to 1 due to rounding.} 
\label{attendrates}
\end{table}

